Brief Announcement: Almost-Tight Approximation Distributed Algorithm for Minimum Cut

In this short paper, we present an improved algorithm for approximating the minimum cut on distributed (CONGEST) networks. Let $\lambda$ be the minimum cut. Our algorithm can compute $\lambda$ exactly in $\tilde{O}((\sqrt{n}+D)\poly(\lambda))$ time, where $n$ is the number of nodes (processors) in the network, $D$ is the network diameter, and $\tilde{O}$ hides $\poly\log n$. By a standard reduction, we can convert this algorithm into a $(1+\epsilon)$-approximation $\tilde{O}((\sqrt{n}+D)/\poly(\epsilon))$-time algorithm. The latter result improves over the previous $(2+\epsilon)$-approximation $\tilde{O}((\sqrt{n}+D)/\poly(\epsilon))$-time algorithm of Ghaffari and Kuhn [DISC 2013]. Due to the lower bound of $\tilde{\Omega}(\sqrt{n}+D)$ by Das Sarma et al. [SICOMP 2013], this running time is {\em tight} up to a $\poly\log n$ factor. Our algorithm is an extremely simple combination of Thorup's tree packing theorem [Combinatorica 2007], Kutten and Peleg's tree partitioning algorithm [J. Algorithms 1998], and Karger's dynamic programming [JACM 2000].

==> one_cut.tex <==
\section{Distributed Algorithm for Finding a Cut that 1-Respects a Tree}\label{sec:one respect tree}

In this section, we solve the following problem: Given a spanning tree $T$ on a network $G$ rooted at some node $r$, we want to find an edge in $T$ such that when we cut it, the cut define by edges connecting the two connected component of $T$ is smallest. To be precise, consider the following definition. \danupon{To do: Define $\cut(X)$.}

\begin{definition}[$v^\downarrow$ and $v^\uparrow$]
For any node $v$ define $v^\downarrow$ to be the set of nodes that are descendants of $v$ in $T$, including $v$. Similarly, define $v^\uparrow$ to be the set of nodes that are ancestors of $v$ in $T$, including $v$. 
\end{definition}

The problem is then to compute 
%
\[c^* = \min_{v\in V(G)} \cut(v^\downarrow).\]
%
%consider any edge $(u, v)$. Let $T_1$ and $T_2$ be the two connected components resulting from cutting $(u, v)$ in $T$. Define $cut_T(u, v)$ be the number of edges between $T_1$ and $T_2$ in $G$. Then, we want to compute $\min_{(u, v)\in E(T)} cut_T(u, v)$. 
%
Below is the main theorem of this section. 
%
\begin{theorem}[Main Result of \Cref{sec:one respect tree}]
There is an $\tilde O(n^{1/2}+D)$-time distributed that can compute $c^*$ as well as find a node $v$ such that  $c^* = \cut(v^\downarrow)$. 
\end{theorem}

%While we state our result as computing the {\em value} of $c^*$, our algorithm will in fact find the cut  

%%We note that our algorithm in facts compute $\cut(v^\downarrow)$ for all $v$ ($v$ knows )

In fact, at the end of our algorithm every node $v$ knows $\cut(v^\downarrow)$. Our algorithm is inspired by Karger's dynamic programming \cite{Karger00}. It relies on the following simple lemma (Lemma 5.9 in \cite{Karger00}). 

%, which says that when we count the degree of all nodes, we will get the value of $\cut(v^\downarrow)$ 

\begin{definition}[$\delta$ and $\rho$]
For any node $v$, let $\delta(v)$ be the weighted degree of $v$, i.e. $\delta(v)=\sum_{u\in V(G)} w(u, v)$. Let $\rho(v)$ denote the total weight of edges whose endpoints' least common ancestor is $v$. Let $\delta^\downarrow(v)=\sum_{u\in v^\downarrow} \delta(u)$ and $\rho^\downarrow(v)=\sum_{u\in v^\downarrow} \rho(u)$. 
\end{definition}

\begin{lemma}[Karger \cite{Karger00}]\label{thm:Karger}
$\cut(v^\downarrow) = \delta^\downarrow(v)-2\rho^\downarrow(v)$.
\end{lemma}

Our algorithm will make sure that every node $v$ knows $\delta^\downarrow(v)$ and $\rho^\downarrow(v)$. By \Cref{thm:Karger}, this will be sufficient for every node $v$ to compute $\cut(v^\downarrow)$. The algorithm is divided in several steps, as presented in the following subsections. 

%... The problem reduces to computing $\delta(u)$ 

%\newcounter{step}
%\addtocounter{step}{1}
%\paragraph{Step \arabic{step}: Partition $T$} 

\danupon{TO DO: Define Diameter}


\begin{figure}
\centering
\begin{subfigure}{0.31\textwidth}
\centering
\includegraphics[page=1, clip=true, trim=7cm 9.9cm 8cm 1.1cm, width=\textwidth]{mincut.pdf}
\caption{}\label{fig:one}
\end{subfigure}
%
\hspace{0.01\textwidth}
%
\begin{subfigure}{0.31\textwidth}
\centering
\includegraphics[page=2, clip=true, trim=7cm 9.9cm 8cm 1.1cm, width=\textwidth]{mincut.pdf}
\caption{}\label{fig:two}
\end{subfigure}
%
\hspace{0.01\textwidth}
%
\begin{subfigure}{0.31\textwidth}
\centering
\includegraphics[page=3, clip=true, trim=7cm 9.9cm 8cm 1.1cm, width=\textwidth]{mincut.pdf}
\caption{}\label{fig:three}
\end{subfigure}

\vspace{0.1cm}

%
\begin{subfigure}{0.31\textwidth}
\centering
\includegraphics[page=4, clip=true, trim=7cm 9.9cm 8cm 1.1cm, width=\textwidth]{mincut.pdf}
\caption{}\label{fig:four}
\end{subfigure}
%
\hspace{0.01\textwidth}
%
\begin{subfigure}{0.31\textwidth}
\centering
\includegraphics[page=5, clip=true, trim=7cm 9.9cm 8cm 1.1cm, width=\textwidth]{mincut.pdf}
\caption{}\label{fig:five}
\end{subfigure}
%
\hspace{0.01\textwidth}
%
\begin{subfigure}{0.31\textwidth}
\centering
\includegraphics[page=6, clip=true, trim=7cm 9.9cm 8cm 1.1cm, width=\textwidth]{mincut.pdf}
\caption{}\label{fig:six}
\end{subfigure}
\caption{\\
(\subref{fig:one}) Graph $G$ with tree $T$ (marked by bold (black) edges) rooted at node of ID $0$ and fragments (defined by triangular regions) obtained from \Cref{subsec:fragment}. \\%
(\subref{fig:two}) Tree $T_F$ (nodes in this tree are the triangles) representing the structure between fragments. This tree is known to every node after we finish the steps in \Cref{subsec:inter fragment tree}.\\ 
(\subref{fig:three}) Tree $T'_F$ representing fragments and their least common ancestors. This tree is known to every node after we finish the steps in\Cref{subsec:LCA of fragments}.}\label{fig:example}
\end{figure}

\subsection{Partition $T$ into Fragments}\label{subsec:fragment}


We partition $T$ into {\em fragments} using the algorithm of Kutten and Peleg \cite{KuttenP98}, which takes $O(n^{1/2}\log^*n+D)$ time. Roughly speaking, this algorithm partitions nodes in tree $T$ into $O(\sqrt{n})$ subtrees, where each subtrees has $O(\sqrt{n})$ diameter (every node knows which edges incident to it are in the subtree containing it). More precisely, Kutten and Peleg showed that one can construct a {\em $(\sqrt{n}+1, O(\sqrt{n})$ spanning forest} in $O(n^{1/2}\log^*n+D)$ time where the notion of spanning forest is as follows. 

\begin{definition}[$(\sigma, \tau)$ spanning forest]\label{def:spanning forest}
A $(\sigma, \tau)$ spanning forest of a graph $G$ is a collection of disjoint trees $\{T_1, \ldots, T_k\}$ with the following properties:
\begin{enumerate}
\item the trees consist of edges of $E$ and span all the nodes of $V$,
\item each tree contains at least $\tau$ nodes, and
\item the diameter of each tree is at most $\tau$. 
\end{enumerate}
\end{definition}

Kutten and Peleg \cite[Section 3.2]{KuttenP98} showed that any tree can be partitioned into a $(k+1, O(k))$ spanning forest in $O(k\log^*k)$ time. We use their algorithm with $k=\sqrt{n}$ to partition tree $T$ into a $(\sqrt{n}+1, O(\sqrt{n}))$ forest\footnote{We note that we in fact do not need this algorithm since we obtain $T$ by using Kutten and Peleg's MST algorithm, which already computes the $(\sqrt{n}+1, O(\sqrt{n}))$ spanning forest as a subroutine. We state their result here for completeness.}. 
%
We use $F_1, \ldots, F_{k+1}$ to denote the resulting fragments.


We can assume that every node in every tree $F_i$ knows the smallest ID among nodes in $F_i$. This can be found in $O(\sqrt{n})$ time by a communication within each fragment. We call such ID an ID of $F_i$, denoted by $\id(F_i)$. We will call a node in $F_i$ whose ID is $\id(F_i)$ {\em a representative node}. 
%
We can further assume that every node knows the IDs of all fragments. This can be done by having the representative node of each fragment broadcast its ID; since there are $O(\sqrt{n})$ fragments, this takes $O(\sqrt{n})$ time. 

\subsection{Compute Inter-Fragment Tree Structure} \label{subsec:inter fragment tree}

We now make every node knows how the fragments are connected (see Fig.~XXX for an example) as follows. Each node $u$ examines each edge in $T$ incident to it. For every edge $(u, v)$ in $T$ such that $v$ is in a different fragment from $u$ ($u$ and $v$ can check this in $O(1)$ time by exchanging the IDs of their fragments), either $u$ or $v$ broadcasts a message $(\id(F_i), \id(F_j))$ where $F_i$ and $F_j$ are fragments that contain $u$ and $v$, respectively. This message represents the fact that fragments $F_i$ and $F_j$ are linked by a tree edge. This step takes $O(\sqrt{n})$ time since there are $O(\sqrt{n})$ edges in $T$ that links between fragments (since there are $O(\sqrt{n})$ fragments). As a result, every node in the graph knows how the fragments are connected by edges in $T$. To be precise, let $T_F$ be a tree where we contract nodes in the same fragment, say $F_i$, into one node which we will call $\id(F_i)$  (see, e.g., Fig.~XXX). The algorithm in this section guarantees that every node knows $T_F$. We call $T_F$ a {\em fragment tree}. We let the root of $T_F$ be the node corresponding to the fragment containing $r$. 


\subsection{Compute Least Common Ancestors of Fragments}\label{subsec:LCA of fragments}

Our goal in this subsection is to identify every node that is the least common ancestor of some pair of fragments, and how these nodes are connected. In particular, we say that a node $v$ is the {\em least common ancestors of fragments} (LCAF) if there are two nodes $x$ and $y$ from different fragments such that 

Consider any fragment $F_i$ having at least two children (i.e.  node $\id(F_i)$ in $T_F$ that has at least two children). 


\subsection{Make Every Node Know Fragments in Its Subtree}\label{subsec:fragment in subtree}

\subsection{Make Every Node Know where It Meats the Fragments}\label{subsec:meet fragments}

\endinput

\paragraph{Step 1: Construct $(\sqrt{n}+1, O(\sqrt{n}))$ spanning forest $F$.} We will assume that we have a $(\sqrt{n}+1, O(\sqrt{n}))$ spanning forest of $G$, denoted by $F$. We can find this in $O(\sqrt{n})$ time, by e.g. treating edges in $T$ as $0$-weight edges (but if we obtain $T$ by packing, we will get this automatically). The property of this spanning forest is that 

\begin{itemize}
\item each tree in the forest is a subtree of $T$, 
\item each tree has radius $O(\sqrt{n})$, 
\item  each tree has at least $\sqrt{n}$ nodes (roughly). 
\end{itemize}

We can find this spanning forest in $O(\sqrt{n})$ time. (See \cite{KuttenP98} in the beginning of Section 5 and Definition 3.1 for details). Note that there are $O(\sqrt{n})$ components.





\paragraph{Step 2: Learn the tree $T$.} At the end of this step, we want every node $v$ to know (1) all edges in $T$ linking between nodes in different component (there are $O(\sqrt{n})$ such edges) and (2) all edges in $T$ linking between nodes in component $C_i$, where $C_i$ is the component that contains $v$. We do the following steps to achieve this. 


\begin{enumerate}

\item[2.1] (Learn inter-component tree-edges) For every edge $(u, v)$ in $T$ that connects two components of $F$, either $u$ or $v$ broadcast this edge to every one. So now every one knows how the components are connected as a tree. This step takes $O(\sqrt{n})$ times since there are $O(\sqrt{n})$ edges linking between $O(\sqrt{n})$ components. 



\item[2.2] (Learn intra-component tree-edges) The ``leader'' of each component $C_i$ counts the number of edges between $C_i$ and $C_j$ in $G$, for all components $C_j$. For each $C_j$, we can do this be upcast. By pipelining, this takes $O(\sqrt{n})$ time in total since $|C_i|=O(\sqrt{n})$. Then, the leader broadcasts these numbers to everyone in $G$ (??? in $F$???). So, every node knows the number of edges between any two components. TO EXPENSIVE.

\end{enumerate}





\endinput

* (cuts w.r.t. inter-component edges) Now we can compute the value of the cut induced by cutting an inter-component edge. Let T' be T with nodes in the same component contracted. Similarly, let G' be G with nodes in the same component contracted. Observe that using information in steps 2 and 3, everyone knows G' and T'. Cutting an inter -component edge is equivalent to cutting the same edge in T'. So, everyone can compute this without communication.

4. (compute m(T_v, C_j)) For each node v in each component C_i, we now want to count the number edges between nodes in the subtree of T rooted at v to other component C_j, denoted by m(T_v, C_j).

4.1 To do this, we figure out the root of C_i which is the node nearest to the root of T. This is easy. Then, everyone in C_i counts the number of edges in its subtree (in C_i only) that link to C_j. This takes O(sqrt(n)) time since the radius of this tree is sqrt(n). We can do this in parallel for all j by pipelining.

4.2 We also compute m(v, x) denoting the number of edges between subtree of v to any node x in C_i (the same component). This can be done by counting upcast again.

4.3 Combining 4.1+4.2, together with the number of inter-component edges between any component C_k that is in the subtree of v and C_j, we can compute m(T_v, C_j). 

* (cuts w.r.t. inside-component edges) To compute the cut when we cut edge (u, v), where u and v are in the same C_i, let's assume that u is nearer to the root of T than v. We we have to know is the number of edge from T_v to all other nodes  outside T_v. This consists of

(1) The number of edges between $latex C_j\subseteq T_v$ to $latex C_k\notin T_v$. This is computed in step 3.

(2) The number of edges between $latex x\in T_v\cap C_i$ to other components  $latex C_k\notin T_v$. This is computed in step 4.1.

(3) The number of edges between $latex x\in T_v\cap C_i$ to other  $latex y\in C_j\setminus T_v$. This is computed in step 4.2.

Since v knows everything we want, it can compute the value of the cut w.r.t. cutting (u, v).
